MEMC-Net: Motion Estimation and Motion Compensation Driven Neural Network for Video Interpolation and Enhancement

Motion estimation (ME) and motion compensation (MC) have been widely used for classical video frame interpolation systems over the past decades. Recently, a number of data-driven frame interpolation methods based on convolutional neural networks have been proposed. However, existing learning based methods typically estimate either flow or compensation kernels, thereby limiting performance on both computational efficiency and interpolation accuracy. In this work, we propose a motion estimation and compensation driven neural network for video frame interpolation. A novel adaptive warping layer is developed to integrate both optical flow and interpolation kernels to synthesize target frame pixels. This layer is fully differentiable such that both the flow and kernel estimation networks can be optimized jointly. The proposed model benefits from the advantages of motion estimation and compensation methods without using hand-crafted features. Compared to existing methods, our approach is computationally efficient and able to generate more visually appealing results. Furthermore, the proposed MEMC-Net can be seamlessly adapted to several video enhancement tasks, e.g., super-resolution, denoising, and deblocking. Extensive quantitative and qualitative evaluations demonstrate that the proposed method performs favorably against the state-of-the-art video frame interpolation and enhancement algorithms on a wide range of datasets.

==> evaluation-figs/Ablation.tex <==
\begin{figure*}[!t]
	\scriptsize
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/beanbags-unet-3.870.png}}
	\scriptsize
	\centerline{(a)  Ours\_noOcc, 3.870 }
\end{minipage}	 
\hfill		
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/beanbags-sepconvlf-3.244.png}}
	\scriptsize
	\centerline{(b) Ours\_SPyNet, 3.244  }
\end{minipage}
\hfill	 
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/beanbags-oursid12661-2.916.png}}
	\scriptsize
	\centerline{(c) Ours\_Small , 2.916 }
\end{minipage}	 	
\hfill		
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/beanbags-gt.png}}
	\scriptsize
	\centerline{(d) Ours  }
\end{minipage}	 
%\vspace{0.1cm}
	
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/walking-unet-2.4810.png}}
	\scriptsize
	\centerline{(e)  Ours\_noOcc, 2.481 }
\end{minipage}	 
\hfill		
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/walking-sepconvlf-2.7715.png}}
		\scriptsize
		\centerline{(f) Ours\_SPyNet, 2.771  }
\end{minipage}
\hfill	 
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/walking-oursid12661_avg2.1625.png}}
		\scriptsize
		\centerline{(g) Ours\_Small , 2.162 }
\end{minipage}	 	
 \hfill		
 \begin{minipage}{0.24\linewidth}
 	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/walking-gt.png}}
 		\scriptsize
 		\centerline{(h) Ours  }
 \end{minipage}	 
%\vspace{0.1cm}
 

\caption{Ablation study of the proposed method.}
% (d) is the pixel-wise region attributions ${R}_t$ montaged on $f_t$ with different graylevels.}
\label{fig:Ablation}

\end{figure*}

==> evaluation-figs/HD720p.tex <==

\begin{figure*}[t]
%	\footnotesize
	\footnotesize
%\tiny
	\centering
	\renewcommand{\tabcolsep}{1pt} % adjust horizontal space
	\renewcommand{\arraystretch}{1} % adjust vertical space
	\begin{center}
		\begin{tabular}{cccccc}
\includegraphics[width=0.16\linewidth]{evaluation-figs/compare_720p_parkrun_6thframe/Toflow/000_IE3.4894_PSNR26.53436.jpg}&
\includegraphics[width=0.16\linewidth]{evaluation-figs/compare_720p_parkrun_6thframe/SepConvlf/parkrun_1280x720_50.yuv_IE2.9975_PSNR26.28785.jpg}&
\includegraphics[width=0.16\linewidth]{evaluation-figs/compare_720p_parkrun_6thframe/SepConvl1/parkrun_1280x720_50.yuv_IE2.7732_PSNR26.60465.jpg}&
\includegraphics[width=0.16\linewidth]{evaluation-figs/compare_720p_parkrun_6thframe/Ours/parkrun_1280x720_50.yuv_IE2.941_PSNR26.69425.jpg}&
\includegraphics[width=0.16\linewidth]{evaluation-figs/compare_720p_parkrun_6thframe/Ours_FWRB/parkrun_1280x720_50.yuv_IE2.9947_PSNR26.66915.png.jpg}&
\includegraphics[width=0.16\linewidth]{evaluation-figs/compare_720p_parkrun_6thframe/GT/parkrun_1280x720_50.yuv_IE0_PSNR48.16835.jpg}\\
			  
(a) ToFlow~\cite{xue2017video}&
(b) SepConv-$L_f$~\cite{niklaus2017videoSepConv}& 
(c) SepConv-$L_1$~\cite{niklaus2017videoSepConv}&
(d) \Ours&
(e) \Ours+&
(f) Ground Truth\\	
	\end{tabular}
	\end{center}
	\vspace{-0.4cm}
\caption{\textbf{Visual comparison on HD videos.}}
\label{fig:720p} %% label for entire figure
%\vspace{-0.2cm}
\end{figure*}


==> evaluation-figs/UCF101.tex <==

\begin{figure*}[t]
%	\footnotesize
	\footnotesize
%\tiny
%\scriptsize
	\centering
	\renewcommand{\tabcolsep}{1pt} % adjust horizontal space
	\renewcommand{\arraystretch}{1} % adjust vertical space
	\begin{center}
		\begin{tabular}{ccccc}
\includegraphics[width=0.195\linewidth]{evaluation-figs/compare_UCF101_2571/Overlay/frame_01_ours_IE4.8713_PSNR19.8131.png}&
\includegraphics[width=0.195\linewidth]{evaluation-figs/compare_UCF101_2571/epicflow/frame_01_ours_epicflow_IE1.9245_PSNR27.4088.png}&
\includegraphics[width=0.195\linewidth]{evaluation-figs/compare_UCF101_2571/SepConvl1/frame_01_ours_IE1.3072_PSNR29.9599.png}&
\includegraphics[width=0.195\linewidth]{evaluation-figs/compare_UCF101_2571/Ours/frame_01_ours_IE1.4604_PSNR33.1329.png}&
\includegraphics[width=0.195\linewidth]{evaluation-figs/compare_UCF101_2571/GT/frame_01_gt_IE0_PSNR48.1329.png}\\
			 	
(a) Overlay&
(b) EpicFlow~\cite{revaud2015epicflow}&
(c) SepConv-$L_1$~\cite{niklaus2017videoSepConv}&
(d) \Ours&
(e) Ground Truth\\				
		\end{tabular}
	\end{center}
	\vspace{-0.4cm}
\caption{\textbf{Visual comparisons on the UCF101 dataset~\cite{soomro2012ucf101}.}}
\label{fig:UCF101} %% label for entire figure
%\vspace{-0.2cm}
\end{figure*}


==> evaluation-figs/denoising.tex <==
\begin{figure*}[!t]
	\scriptsize
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/beanbags-unet-3.870.png}}
	\scriptsize
	\centerline{(a)  MIND~\cite{long2016learning}, 3.870 }
\end{minipage}	 
\hfill		
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/beanbags-sepconvlf-3.244.png}}
	\scriptsize
	\centerline{(b) SepConv~\cite{niklaus2017videoSepConv}, 3.244  }
\end{minipage}
\hfill	 
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/beanbags-oursid12661-2.916.png}}
	\scriptsize
	\centerline{(c) Ours, 2.916 }
\end{minipage}	 	
\hfill		
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/beanbags-gt.png}}
	\scriptsize
	\centerline{(d) Groundtruth  }
\end{minipage}	 
%\vspace{0.1cm}
	
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/walking-unet-2.4810.png}}
	\scriptsize
	\centerline{(e)  MIND~\cite{long2016learning}, 2.481 }
\end{minipage}	 
\hfill		
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/walking-sepconvlf-2.7715.png}}
		\scriptsize
		\centerline{(f) SepConv~\cite{niklaus2017videoSepConv}, 2.771  }
\end{minipage}
\hfill	 
\begin{minipage}{0.24\linewidth}
	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/walking-oursid12661_avg2.1625.png}}
		\scriptsize
		\centerline{(g) Ours, 2.162 }
\end{minipage}	 	
 \hfill		
 \begin{minipage}{0.24\linewidth}
 	\centerline{\includegraphics[width= 1.0\textwidth]{preface-compare/walking-gt.png}}
 		\scriptsize
 		\centerline{(h) Groundtruth  }
 \end{minipage}	 
%\vspace{0.1cm} 
\caption{Visual comparisons of video interpolation methods.}
% (d) is the pixel-wise region attributions ${R}_t$ montaged on $f_t$ with different graylevels.}
\label{fig:denoising}

\end{figure*}

==> evaluation-speed/running-speed.tex <==
\begin{table}[!t]

\caption{Runtime speed for different methods on 480p, 720p and 1080p format images. The runtime on $640 \times 480$p image is obtained from Middlebury~\cite{baker2011database} benchmark (except for ToFlow~\cite{xue2017video}), where every method reports its speed on the \textit{Urban} sequence.}
\label{tab:running-speed}
\scriptsize
%%\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.8cm}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand{\setTableWid}{ m{9pt}<{\centering} }
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\centering
\begin{tabular}{m{2.5cm}  P{2.0cm} P{2.0cm} P{2.0cm}   }
\toprule
%\multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} & \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}
%\multirow{1}{*}{  Methods} &\multicolumn{2}{c}{Vimeo90K~\cite{xue2017video}} \\
%\cmidrule{2-3}
%\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}
Methods & $640 \times 480$p& $1280 \times 720$p &$1920 \times 1080$p 	 \\
\midrule
AdaConv~\cite{niklaus2017videoAdaConv}  & 2.80s & --- &  ---\\
SuperSlomo~\cite{jiang2017super} &0.50s	 & --- & ---\\ 
ToFlow~\cite{xue2017video} & 0.43s & 1.01s & 1.90s\\
SepConv~\cite{niklaus2017videoSepConv}  &0.20s   & 0.50s & 0.90s \\
%%\Ours\_SpyNet& &&&&&& 15,857,951 \\
%\Ours\_Small &  &&&&&&7,204,367 \\ 
%\Ours\_SpyNet & 0.13s & 0.34s &0.68\\
\Ours\_Small & 0.13s & 0.33s& 0.67s\\
\Ours   & \first{0.06s} & \first{0.20s} & \first{0.41s}\\
%\midrule
\bottomrule
\end{tabular} 

\end{table}

==> evaluation-tables/MiddleBury.tex <==
\begin{table*}[!t]
 
 \caption{Evaluation on the MiddleBury benchmark dataset. The \textit{disc.} represents discontinuous motion region and the \textit{unt.} represents texture-less region. }
 \label{tab:MiddleBury}
% \scriptsize/
 \tiny
%%\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.8cm}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand{\setTableWid}{ m{9pt}<{\centering} }
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\centering
\begin{tabular}{m{1.5cm}  P{0.4cm}P{0.4cm}P{0.4cm} P{0.4cm}P{0.4cm}P{0.4cm}  P{0.4cm}P{0.4cm}P{0.4cm}  P{0.4cm}P{0.4cm}P{0.4cm}  P{0.4cm}P{0.4cm}P{0.4cm}  P{0.4cm}P{0.4cm}P{0.4cm}  P{0.4cm}P{0.4cm}P{0.4cm}  P{0.4cm}P{0.4cm}P{0.4cm}  P{0.4cm}P{0.4cm}P{0.4cm}   }
\toprule
%\multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} & \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}
\multirow{2}{*}{Methods} &  \multicolumn{3}{c}{Mequon}&  \multicolumn{3}{c}{Schefflera }&  \multicolumn{3}{c}{Urban }&  \multicolumn{3}{c}{Teddy }&  \multicolumn{3}{c}{Backyard}&  \multicolumn{3}{c}{Basketball}&  \multicolumn{3}{c}{ Dumptruck }&  \multicolumn{3}{c}{Evergreen }&  \multicolumn{3}{c}{AVERAGE} \\
\cmidrule{2-9}
%\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}
	&all &\textit{disc.} & \textit{unt.} & all &\textit{disc.} & \textit{unt.} &all &\textit{disc.} & \textit{unt.} &all &\textit{disc.} & \textit{unt.} &all &\textit{disc.} & \textit{unt.} &all &\textit{disc.} & \textit{unt.} &all &\textit{disc.} & \textit{unt.} &all &\textit{disc.} & \textit{unt.} &all &\textit{disc.} & \textit{unt.}  \\
\midrule


MDP-Flow2~\cite{xu2012motion} 				&2.89 	&5.38 	&1.19 	&3.47 	&5.07 	&1.26 	&3.66 	&6.10 	&2.48 	&5.20 	&7.48 	&3.14 	&10.20 	&12.80 	&3.61 	&6.13 	&11.80 	&2.31 	&7.36 	&16.80 	&1.49 	&7.75 	&12.10 	&1.69 	&5.83 	&9.69 	&2.15 \\
DeepFlow2~\cite{weinzaepfel2013deepflow}	&2.98 	&5.67 	&1.22 	&3.88 	&5.78 	&1.52 	&3.62 	&5.93 	&1.34 	&5.39 	&7.20 	&3.17 	&11.00 	&13.90 	&3.63 	&5.91 	&11.30 	&2.29 	&7.14 	&16.30 	&1.49 	&7.80 	&12.20 	&1.70 	&5.97 	&9.79 	&2.05 \\
SuperSlomo~\cite{jiang2017super}			&2.51 	&4.32 	&1.25 	&3.66 	&5.06 	&1.93 	&2.91 	&4.00 	&1.41 	&5.05 	&6.27 	&3.66 	&9.56 	&11.90 	&3.30 	&5.37 	&10.20 	&2.24 	&6.69 	&15.00 	&1.53 	&6.73 	&10.40 	&1.66 	&5.31 	&8.39 	&2.12 \\
SepConv (l1)~\cite{niklaus2017videoSepConv} &2.52 	&4.83 	&1.11 	&3.56 	&5.04 	&1.90 	&4.17 	&4.15 	&2.86 	&5.41 	&6.81 	&3.88 	&10.20 	&12.80 	&3.37 	&5.47 	&10.40 	&2.21 	&6.88 	&15.60 	&1.72 	&6.63 	&10.30 	&1.62 	&5.61 	&8.74 	&2.33 \\
Ours (\Ours)									&2.83 	&5.28 	&1.31 	&3.84 	&5.31 	&1.94 	&4.16 	&4.27 	&2.20 	&5.75 	&7.49 	&3.94 	&8.57 	&10.60 	&3.25 	&4.99 	&9.42 	&2.14 	&5.86 	&13.10 	&1.60 	&6.83 	&10.70 	&1.57 	&5.35 	&8.27 	&2.24 \\
%
%%EpicFlow~\cite{revaud2015epicflow} &33.71 & 0.9635 &32.02&0.9622& ---& 6.48 & ---& ---\\
%MDP-Flow2~\cite{xu2012motion} 
%DeepFlow~\cite{weinzaepfel2013deepflow}
%%DeepFlow2~\cite{revaud2015deep} 
%%PMMST~\cite{Zhang2015High} 
%SuperSlomo~\cite{jiang2017super}
%%SepConv (lf)~\cite{niklaus2017videoSepConv} & 34.69 & 0.9655  & 33.45& 0.9674& 2.44& --- & 33.37 & 0.9336\\
%SepConv (l1)~\cite{niklaus2017videoSepConv} & 34.78 & 0.9669  &33.79& \textbf{0.9702}& 2.27 & 5.605 &\textbf{33.78}&\textbf{0.9398}\\
%Ours & \textbf{34.94 } & \textbf{0.9675 } &\textbf{33.86}& 0.9688 &\textbf{2.23} & ? &33.59&0.9323\\

\bottomrule
\end{tabular} 

\end{table*}

==> evaluation-tables/cif.tex <==
\begin{table*}[!t]
 
 \caption{Evaluation on CIF format (352$\times$288) videos.}
 \label{tab:cif}
 \scriptsize
 
%%\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.8cm}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand{\setTableWid}{ m{9pt}<{\centering} }
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\centering
\begin{tabular}{m{1.5cm}  P{0.68cm} P{0.68cm}  P{0.68cm} P{0.68cm}  P{0.68cm}P{0.68cm} P{0.68cm}  P{0.68cm} P{0.68cm} P{0.68cm} P{0.68cm} P{0.68cm} P{0.68cm}  }
\toprule
%\multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} & \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}
\multirow{1}{*}{Methods} & Akiyo&Bus&City&\tabincell{c}{Coast-\\guard}&\tabincell{c}{Conta-\\iner}&Flower&\tabincell{c}{Foot-\\ball}&\tabincell{c}{Fore-\\man} & Hall & \tabincell{c}{Mobi-\\le} &News &Silent &Soccer\\ 
%\cmidrule{2-7}
%\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}%	interp. error & interp. error \\
%  Ice MobileNews Paris Silent Soccer Stefan
%Water& News Paris Silent Soccer Stefan 
%-fall
%&&&&&&&&&&\\
\midrule
%SpyNet~\cite{ranjan2017optical} & 33.67 & 0.9633 &31.95 & 0.9601& ---& ---\\
%EpicFlow~\cite{revaud2015epicflow} &33.71 & 0.9635 &32.02&0.9622& ---& ? \\
%ToFlow~\cite{xue2017video} & 34.54 & 0.9666 &33.53 &0.9668& --- & --- \\
MIND~\cite{long2016learning}&42.10 &26.25 &33.63 &32.97&37.39&27.81&\textbf{23.14}&32.63&35.88&28.01&34.29&34.69&\textbf{27.38} \\
Toflow~\cite{xue2017video} &44.46&25.46&\textbf{35.14}&34.04&41.51&31.18&22.24&32.75&36.1&\textbf{30.13}&35.00&35.19&26.69\\
SepConv~\cite{niklaus2017videoSepConv}&45.72&25.40&34.78&33.35&42.33&31.95&22.23&33.20&36.24&30.61&34.79&35.40&26.99\\
%SepConv (l1)~\cite{niklaus2017videoSepConv} & 34.78 & 0.9669  &33.79& \textbf{0.9702}& 2.27 &?\\
%Ours &46.03 &25.37&34.93&33.94&42.53&32.07&22.81&33.52&36.44&32.70&29.94&35.05&35.84&27.14\\
Ours &\textbf{46.04}&\textbf{25.41}&35.11&\textbf{34.04}&\textbf{42.55}&\textbf{32.20}&22.81&\textbf{33.56}&\textbf{36.46}&30.06&\textbf{35.06}&\textbf{35.85}&27.17\\

\bottomrule
\end{tabular} 

\end{table*}

==> evaluation-tables/denoising.tex <==
\begin{table}[!t]


\caption{Evaluation  results of video denoising.}
\label{tab:denoising}
\scriptsize
%%\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.8cm}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand{\setTableWid}{ m{9pt}<{\centering} }
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\centering
\begin{tabular}{m{2.5cm}  P{1.0cm} P{1.0cm}  }
\toprule
%\multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} & \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}
\multirow{2}{*}{  Methods} &\multicolumn{2}{c}{Vimeo90K~\cite{xue2017video}} \\
\cmidrule{2-3}
%\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}
&PSNR & SSIM 	 \\
\midrule
ToFlow~\cite{xue2017video} & 28.85 & 0.9407 \\
%%Ours\_SpyNet& &&&&&& 15,857,951 \\
Ours\_Small &  &&&&&&7,204,367 \\ 
Ours(8500)   & &\\

\bottomrule
\end{tabular} 


\caption{Evaluation results of video denoising.}
\label{tab:deblock}
\scriptsize
%%\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.8cm}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand{\setTableWid}{ m{9pt}<{\centering} }
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\centering

\begin{tabular}{m{2.5cm}  P{1.0cm} P{1.0cm}  }
\toprule
%\multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} & \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}
\multirow{2}{*}{  Methods} &\multicolumn{2}{c}{Vimeo90K~\cite{xue2017video}} \\
\cmidrule{2-3}
%\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}
&PSNR & SSIM 	 \\
\midrule
ToFlow~\cite{xue2017video} & 28.85 & 0.9407 \\
%%Ours\_SpyNet& &&&&&& 15,857,951 \\
Ours\_Small &  &&&&&&7,204,367 \\ 
Ours(8500)   & &\\

\bottomrule
\end{tabular} 
\end{table}

==> evaluation-tables/kernelbased4.tex <==
\begin{table*}[!t]
 
 \caption{Evaluation on the UCF101, Vimeo90K and MiddleBury datasets.}
 \label{tab:denoising}
%\scriptsize
\footnotesize
%%\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.8cm}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand{\setTableWid}{ m{9pt}<{\centering} }
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\centering
\begin{tabular}{m{2.5cm}  P{1.0cm} P{1.0cm}  P{1.0cm} P{1.0cm}  P{1.5cm} P{1.5cm}  r}
\toprule
%\multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} & \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}
\multirow{2}{*}{  Methods} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}} &\multicolumn{2}{c}{Vimeo90K~\cite{xue2017video}} &MiddleBury (Other)~\cite{baker2011database}
&MiddleBury (Eval)~\cite{baker2011database} &\multirow{2}{*}{\tabincell{c}{\#Num. of \\ Parameters}}   \\
\cmidrule{2-7}
%\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}
	&PSNR & SSIM 	&PSNR & SSIM	& 
	interp. error & interp. error & \\
\midrule
Ours\_noOcc & &&&&&& \\
Ours\_SpyNet& &&&&&& 15,857,951 \\
Ours\_Small &  &&&&&&7,204,367 \\ 
Ours & \textbf{34.94 } & \textbf{0.9675 } &\textbf{33.86}& 0.9688 &\textbf{2.23} & ?& 53,077,987\\

\bottomrule
\end{tabular} 

\end{table*}

==> evaluation-tables/progressiveflow.tex <==
\begin{table*}[!t]
 
 \caption{\textbf{Analysis of interpolation error with respect to flow magnitude.}}
 \label{tab:progressiveflow}
% \scriptsize
\tiny
%%\setlength{\abovecaptionskip}{0.cm}
%\setlength{\belowcaptionskip}{-0.8cm}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand{\setTableWid}{ m{9pt}<{\centering} }
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\centering
\begin{tabular}{m{1.8cm}  P{1.0cm}P{1.3cm}P{0.6cm}P{0.6cm} P{0.8cm} P{0.8cm}  P{0.8cm} P{0.8cm} P{1.6cm}  r}
\toprule
%\multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} & \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}
\multirow{2}{*}{  Methods}& \multicolumn{4}{c}{Subnetworks} &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}} &\multicolumn{2}{c}{Vimeo90K~\cite{xue2017video}} &Middlebury~\cite{baker2011database}
 &\multirow{2}{*}{\tabincell{c}{\#Param.}}   \\
\cmidrule(l{2pt}r{2pt}){2-5} 
\cmidrule(l{2pt}r{2pt}){6-7}
\cmidrule(l{2pt}r{2pt}){8-9} 
\cmidrule(l{2pt}r{2pt}){10-10}

%\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}
&flow& kernel (size)& occ. & enh.	&PSNR & SSIM 	&PSNR & SSIM	& 
IE \tiny{(oth.)}& \\
\midrule
SepConv-$L_f$~\cite{niklaus2017videoSepConv} & $\times$  &learned (51) & $\times$ & $\times$ & 34.69 & 0.9655  & 33.45& 0.9674& 2.44 &21,675,452\\
SepConv-$L_1$~\cite{niklaus2017videoSepConv} &$\times$  &learned (51) & $\times$ & $\times$ & 34.78 & 0.9669  &33.79& \first{0.9702}& 2.27& 21,675,452 \\
\midrule
\multirow{3}{*}{Ours}
%Ours\_onlyFilter 
&$\times$ &learned (4) & $\times$ & $\times$ & 34.89 &\first{0.9682} &32.73& 0.9581 &2.74& 14,710,415\\
%Ours\_Filter\&Enh 
&$\times$ &learned (4) & $\times$ & $\surd$ & \first{34.97} &\first{0.9682}&33.31& 0.9633& 2.57& 14,720,783\\
%Ours\_ks51 (9013) & &&&&& 14,919,871\\
%Ours 
&FlowNetS &learned (4) & $\surd$ & $\surd$ & \second{34.94} & \second{0.9675} &\first{33.86}& 0.9693 &\first{2.23} & 53,077,987\\

\bottomrule
\end{tabular} 

\end{table*}

==> net-arch/MEMC_arch.tex <==
\begin{figure}[!t]
	\setlength{\belowcaptionskip}{-0.cm}
	\centering	
	\begin{minipage}{0.9\linewidth}
		\centering{	 \includegraphics[width= 1.0\textwidth]{net-arch/MEMC_arch.pdf}}
	\end{minipage}
	
	\caption{\textbf{Conventional MEMC framework.}
	 }
	\label{fig:MEMC_arch}
\end{figure}

==> net-arch/flow-project.tex <==
\begin{figure}[!t]
	
%		\setlength{\abovecaptionskip}{0.cm}
%		\setlength{\belowcaptionskip}{-0.cm}
	\centering	
%%	\begin{minipage}{0.40\linewidth}
%		\centering{	 \includegraphics[width= 1.0\textwidth]{net-arch/flow-project.png}}
%	\end{minipage}
%	\hfill
	\begin{minipage}{0.45\linewidth}
		\centering{	 \includegraphics[width= 0.8\textwidth]{net-arch/flow_project_1.pdf}}
	\end{minipage}
	%$\hat{\mathrm{x}}^{1}$, $\hat{\mathrm{x}}^{2}$ and $\hat{\mathrm{x}}^{3}$
	\vspace{-5pt}
	\caption{\textbf{Proposed flow projection layer.} %\jason{This figure is of low quality. Could you use pdf file instead?}
	 }
	 \vspace{-8pt}
	\label{fig:flow-project}
%		\setlength{\abovecaptionskip}{0.0cm}
%		\setlength{\belowcaptionskip}{0.2cm}
\end{figure}
